A Benchmark for Generalizable and Interpretable Temporal Question Answering over Knowledge Bases

Knowledge Base Question Answering (KBQA) tasks that involve complex reasoning are emerging as an important research direction. However, most existing KBQA datasets focus primarily on generic multi-hop reasoning over explicit facts, largely ignoring other reasoning types such as temporal, spatial, and taxonomic reasoning. In this paper, we present a benchmark dataset for temporal reasoning, TempQA-WD, to encourage research in extending the present approaches to target a more challenging set of complex reasoning tasks. Specifically, our benchmark is a temporal question answering dataset with the following advantages: (a) it is based on Wikidata, which is the most frequently curated, openly available knowledge base, (b) it includes intermediate sparql queries to facilitate the evaluation of semantic parsing based approaches for KBQA, and (c) it generalizes to multiple knowledge bases: Freebase and Wikidata. The TempQA-WD dataset is available at https://github.com/IBM/tempqa-wd.

==> text/data/analysis.tex <==
\subsection{Dataset Analysis}


==> text/data/wikidata.tex <==
\subsection{Wikidata}
Wikidata\footnote{https://www.wikidata.org/} is a free knowledge base that is actively updated and maintained. It has 93.65 million data items as of May, 2021 and continuously growing each day with permission for volunteers to edit and add new data items. We chose Wikidata as our knowledge base as it has many temporal facts with appropriate knowledge representation encoded. %embedded with the statements in the form of reified statements, making it an interesting KB for testing temporal question answering. 
It supports reification of statements (triples) to add additional metadata with qualifiers such as start date, end date, point in time, location ... etc. 
%to capture valid time interval of the statement, location where the event has occurred or any other details that are relevant to the system. 
This makes it an interesting choice to build benchmark datasets to test different kinds of reasoning including temporal reasoning.

==> text/eval/datasets.tex <==
\subsection{Datasets}
\label{sec:data}

%\begin{table}[htb]
%\begin{center}
%\small
%\begin{tabular}{|l|ll|}
%\hline
%  Dataset  & Dev & Test  \\
%\hline
% TempQA-WD   &    175       & 664       \\
%SWQ-WD &  200       & 5622       \\
% WebQSP-WD &       200     & 1033   \\
%\hline
%\end{tabular}
%\caption{Datasets }
%\label{table:datasets}
%\end{center}
%\end{table}
Along with the new benchmark dataset \dataset~introduced in this paper, we also evaluate our baseline system on two other benchmark datasets adopted to Wikidata, to evaluate its effectiveness beyond temporal questions. They are SWQ-WD%\footnote{https://github.com/askplatypus/wikidata-simplequestions}
~\cite{wikidata-benchmark}, WebQSP-WD
%\footnote{https://github.com/UKPLab/coling2018-graph-neural-networks-question-answering}
~\cite{C18-1280}.
Dev/test sizes of SWQ-WD 200/5622, WebQSP-WD 200/1033. 
%Table~\ref{table:datasets} gives the details of dev and test splits used. 
The baseline system is tuned with dev sets of TempQA-WD and SWQ-WD, and evaluated on all the three test datasets. %As pointed by the authors of WebQSP-WD, the dataset is not validated to verify if the question is answerable on Wikidata and if the gold answers are up-to-date with respect Wikidata answers. Our analysis on a subset of $200$ dev questions found that $85$ of the questions had ground truth issue with respect to Wikidata.
%with either answer being different as per Wikidata or more answers being present than what came from Freebase or supporting facts not being present in the Wikidata to answer them. Performance on this dataset need to be interpreted keeping this issue in mind.


